Constrained C-Test Generation via Mixed-Integer Programming

This work proposes a novel method to generate C-Tests; a deviated form of cloze tests (a gap filling exercise) where only the last part of a word is turned into a gap. In contrast to previous works that only consider varying the gap size or gap placement to achieve locally optimal solutions, we propose a mixed-integer programming (MIP) approach. This allows us to consider gap size and placement simultaneously, achieving globally optimal solutions, and to directly integrate state-of-the-art models for gap difficulty prediction into the optimization problem. A user study with 40 participants across four C-Test generation strategies (including GPT-4) shows that our approach (MIP) significantly outperforms two of the baseline strategies (based on gap placement and GPT-4); and performs on-par with the third (based on gap size). Our analysis shows that GPT-4 still struggles to fulfill explicit constraints during generation and that MIP produces C-Tests that correlate best with the perceived difficulty. We publish our code, model, and collected data consisting of 32 English C-Tests with 20 gaps each (totaling 3,200 individual gap responses) under an open source license.

==> images/gap_size.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4818.00,2550.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,734){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(592,957){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(592,1179){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \put(592,1402){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(592,1624){\makebox(0,0)[r]{\strut{}$2.5$}}%
      \put(592,1847){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(592,2069){\makebox(0,0)[r]{\strut{}$3.5$}}%
      \put(688,352){\makebox(0,0){\strut{}$0$}}%
      \put(1072,352){\makebox(0,0){\strut{}$0.1$}}%
      \put(1456,352){\makebox(0,0){\strut{}$0.2$}}%
      \put(1840,352){\makebox(0,0){\strut{}$0.3$}}%
      \put(2224,352){\makebox(0,0){\strut{}$0.4$}}%
      \put(2609,352){\makebox(0,0){\strut{}$0.5$}}%
      \put(2993,352){\makebox(0,0){\strut{}$0.6$}}%
      \put(3377,352){\makebox(0,0){\strut{}$0.7$}}%
      \put(3761,352){\makebox(0,0){\strut{}$0.8$}}%
      \put(4145,352){\makebox(0,0){\strut{}$0.9$}}%
      \put(4529,352){\makebox(0,0){\strut{}$1$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(152,1290){\rotatebox{-270}{\makebox(0,0){\strut{}Average Gap Size}}}%
      \put(2608,112){\makebox(0,0){\strut{}$	au$}}%
      \put(2608,2309){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%%
      \put(1585,788){\makebox(0,0)[r]{\strut{}MIP$_{\text{BERT}}$}}%
      \csname LTb\endcsname%%
      \put(1585,628){\makebox(0,0)[r]{\strut{}MIP$_{\text{no-BERT}}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,734){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(592,957){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(592,1179){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \put(592,1402){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(592,1624){\makebox(0,0)[r]{\strut{}$2.5$}}%
      \put(592,1847){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(592,2069){\makebox(0,0)[r]{\strut{}$3.5$}}%
      \put(688,352){\makebox(0,0){\strut{}$0$}}%
      \put(1072,352){\makebox(0,0){\strut{}$0.1$}}%
      \put(1456,352){\makebox(0,0){\strut{}$0.2$}}%
      \put(1840,352){\makebox(0,0){\strut{}$0.3$}}%
      \put(2224,352){\makebox(0,0){\strut{}$0.4$}}%
      \put(2609,352){\makebox(0,0){\strut{}$0.5$}}%
      \put(2993,352){\makebox(0,0){\strut{}$0.6$}}%
      \put(3377,352){\makebox(0,0){\strut{}$0.7$}}%
      \put(3761,352){\makebox(0,0){\strut{}$0.8$}}%
      \put(4145,352){\makebox(0,0){\strut{}$0.9$}}%
      \put(4529,352){\makebox(0,0){\strut{}$1$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(152,1290){\rotatebox{-270}{\makebox(0,0){\strut{}Average Gap Size}}}%
      \put(2608,112){\makebox(0,0){\strut{}$	au$}}%
      \put(2608,2309){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%%
      \put(2738,788){\makebox(0,0)[r]{\strut{}SEL}}%
      \csname LTb\endcsname%%
      \put(2738,628){\makebox(0,0)[r]{\strut{}SEL$_{\text{XBG}}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(592,512){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(592,734){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(592,957){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(592,1179){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \put(592,1402){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(592,1624){\makebox(0,0)[r]{\strut{}$2.5$}}%
      \put(592,1847){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(592,2069){\makebox(0,0)[r]{\strut{}$3.5$}}%
      \put(688,352){\makebox(0,0){\strut{}$0$}}%
      \put(1072,352){\makebox(0,0){\strut{}$0.1$}}%
      \put(1456,352){\makebox(0,0){\strut{}$0.2$}}%
      \put(1840,352){\makebox(0,0){\strut{}$0.3$}}%
      \put(2224,352){\makebox(0,0){\strut{}$0.4$}}%
      \put(2609,352){\makebox(0,0){\strut{}$0.5$}}%
      \put(2993,352){\makebox(0,0){\strut{}$0.6$}}%
      \put(3377,352){\makebox(0,0){\strut{}$0.7$}}%
      \put(3761,352){\makebox(0,0){\strut{}$0.8$}}%
      \put(4145,352){\makebox(0,0){\strut{}$0.9$}}%
      \put(4529,352){\makebox(0,0){\strut{}$1$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(152,1290){\rotatebox{-270}{\makebox(0,0){\strut{}Average Gap Size}}}%
      \put(2608,112){\makebox(0,0){\strut{}$	au$}}%
      \put(2608,2309){\makebox(0,0){\strut{} }}%
      \csname LTb\endcsname%%
      \put(3890,788){\makebox(0,0)[r]{\strut{}SIZE}}%
      \csname LTb\endcsname%%
      \put(3890,628){\makebox(0,0)[r]{\strut{}SIZE$_{\text{XGB}}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{images/gap_size.eps}}%
    \gplfronttext
  \end{picture}%
\endgroup

